Classifica\c{c}\~ao de esp\'ecies de peixe utilizando redes neurais convolucional

Data classification is present in different real problems, such as recognizing patterns in images, differentiating defective parts in a production line, classifying benign and malignant tumors, among many others. Many of these problems have data patterns that are hard to identify, which requires more advanced techniques for resolution. Recently, several works addressing different artificial neural network architectures have been applied to solve classification problems. When the classification problem must be obtained through images, currently, the standard methodology is the use of convolutional neural networks. Thus, in this report convolutional neural networks are used to classify fish species. Classifica\c{c}\~ao de dados est\'a presente em diversos problemas reais, tais como: reconhecer padr\~oes em imagens, diferenciar pe\c{c}as defeituosas em uma linha de produ\c{c}\~ao, classificar tumores benignos e malignos, dentre diversas outras. Muitos desses problemas possuem padr\~oes de dados dif\'iceis de serem identificados, o que requer, consequentemente, t\'ecnicas mais avan\c{c}adas para sua resolu\c{c}\~ao. Recentemente, diversos trabalhos abordando diferentes arquiteturas de redes neurais artificiais v\^em sendo aplicados para solucionar problemas de classifica\c{c}\~ao. Quando a classifica\c{c}\~ao do problema deve ser obtida por meio de imagens, atualmente a metodologia padr\~ao \'e uso de redes neurais convolucionais. Sendo assim, neste trabalho s\~ao utilizadas redes neurais convolucionais para classifica\c{c}\~ao de esp\'ecies de peixes.

==> src/mult-mat.tex <==
Nesta seção, é realizada uma discussão da metodologia de multiplicação de matrizes utilizado GPU e OpenMP com CPU. Recapitulando brevemente a multiplicação de matrizes, supõe-se que deseja-se multiplicar as matrizes $A_{m \times n}$ por $B_{n \times w}$. O resultado dessa operação sera uma matriz $C_{m \times w}$, ou seja, $A \times B = C$. A Figura \ref{fig:exmatmul} mostra de maneira intuitiva a ideia por trás da multiplicação de matrizes. Para se obter os elementos de $C$, cada linha de $A$ é multiplicada elemento a elemento por uma coluna de $B$. Ao final o valor é agregado por meio de um somatório. É importante ressaltar que para a multiplicação ser viável, o número de colunas de $A$ deve ser igual ao número de linhas de $B$.

\begin{figure}[h]
\centering
\includegraphics[scale=0.2]{figuras/matmult.png}
\caption{Exemplo de multiplicação de matrizes com uma matriz 2 x 2}
\label{fig:exmatmul}
\end{figure}

\noindent Dessa maneira é fácil observar que multiplicar matrizes é um bom exemplo de computação paralela. Cada elemento de $C$ é computado de maneira independente, logo, pode ser paralelizado.

\subsection{Multiplicando matrizes na GPU}
A primeira abordagem para paralelização da multiplicação de matrizes utilizando uma GPU é disparar diversas \textit{threads} fazendo com que cada uma calcule um elemento da matriz resultante $C$. Nesta abordagem, cada \textit{thread} ler uma linha de $A$ e uma coluna de $B$ para computar o elemento $c_{ij}$ de $C$, sendo $i = 1 \cdots  m$ e $j = 1 \cdots  w$. Na Figura \ref{fig:multabs1} é ilustrada essa abordagem \cite{manualCUDA}. Utilizando essa abordagem de multiplicação, as matrizes $A$ e $B$ são é carregadas na memória global $w$ e $m$ vezes, respectivamente. Com isso o algoritmo faz muitos acessos à memória global, que possui alta latência e baixo \textit{throughput}. 

\begin{figure}[h]
\centering
\includegraphics[scale=0.45]{figuras/mult_abd1.png}
\caption{Multiplicação de matrizes na qual cada \textit{thread} calcula $c_{ij}$} 
\label{fig:multabs1}
\end{figure}

Com intuito de extrair a eficiência máxima que uma GPU pode entregar, a segunda abordagem de multiplicação de matrizes na GPU tem como objetivo utilizar a memória compartilhada de cada bloco de \textit{threads} visando reduzir o número de acessos a memória global do dispositivo. Para isso as matrizes são subdivididas em pequenos blocos como mostrado na Figura \ref{fig:multabs2} \cite{manualCUDA}. Essa técnica é conhecida como multiplicação por ladrilhamento e diferentemente da abordagem anterior, no qual toda linha de $A$ e coluna $B$ era multiplicada de uma só vez gerando assim um elemento de $C$, no ladrilhamento tem-se submatrizes de $A$ e $B$ que vão gerar um valor parcial de um elemento de $C$. Quando todos os ladrilhos forem processados o valor final de cada um dos elementos da matriz $C$ será o somatório de cada elemento parcial obtido pela multiplicação de cada uma das linhas e colunas submatrizes $A$ e $B$, respectivamente.

\begin{figure}[h]
\centering
\includegraphics[scale=0.45]{figuras/mult_abd2.png}
\caption{Multiplicação de matrizes utilizando ladrilhamento} 
\label{fig:multabs2}
\end{figure}

O objetivo de principal de se usar o ladrilhamento em GPU é carregar cada submatriz na memória compartilhada do bloco de \textit{threads}. O caso ideal seria alocar toda matriz dentro de uma memória compartilhada. Porém, como já mencionado, essa memória é de tamanho reduzido quando comparada com a memória global. Dessa forma, a ideia é carregar na memória compartilhada apenas submatrizes de $A$ e $B$, na qual cada bloco de \textit{threads} pode compartilhar seus dados de maneira rápida. Com isso, um requisito de projeto é que o ladrilho caiba dentro de um bloco de \textit{threads} da GPU. O valor do tamanho do bloco varia de acordo com o dispositivo e cabe ao programador conhecer a arquitetura para melhor aproveitá-la.

Fazendo uma breve comparação entre as duas abordagens de multiplicação de matrizes em GPU apresentadas anteriormente, a Figura \ref{fig:complad} apresenta um gráfico de tempo de execução de cada um dos métodos em relação a ordem das matrizes multiplicadas. É possível observar o ganho de performance na medida que as matrizes aumentam. A arquitetura utilizada para gerar este gráfico será discutida na seção IV. 

\begin{figure}[h]
\centering
\includegraphics[scale=0.6]{figuras/comp_GPUc.png}
\label{fig:complad}
\caption{Comparação entre as abordagens com e sem ladrilhamento na GPU utilizando precisão simples. As matrizes A e B são quadradas e os tamanhos são indicados no gráfico} 
\label{fig:complad}
\end{figure}

\subsection{Multiplicando matrizes na CPU com OpenMP}
A ideia de ladrilhamento das matrizes, discutida na seção anterior, também aplicada na CPU. Na GPU, as \textit{threads} são disparadas e com os índices de cada uma delas é possível operar sobre os dados de acordo com seus blocos. Na CPU esses índices são obtidos por loops de controle. O objetivo principal do ladrilhamento também é o mesmo: tirar proveito da arquitetura de CPU através da memória cache de acesso rápido. Mesmo no código sequencial já se obtém um ganho de performance, como mostrado na Figura \ref{fig:complad2}

\begin{figure}[h]
\centering
\includegraphics[scale=0.6]{figuras/comp_CPUc.png}
\caption{Comparação entre as abordagens com e sem ladrilhamento na CPU para precisão simples. As matrizes A e B são quadradas e os tamanhos são indicados no gráfico}
\label{fig:complad2}
\end{figure}

Para realizar paralelização por meio da CPU é utilizado a OpenMP. A API dá suporte as linguagens C/C++ e Fortran, e basicamente o que deve ser incluído ao código original são diretiva em trechos de códigos que devem ser paralelizado. Com isso, a API é capaz de disparar \textit{threads} utilizando os núcleos da CPU em questão. Um exemplo de diretiva para paralelizar um loop em C é descrito a seguir:

\begin{verbatim}
#pragma omp parallel for default(none) \
  shared(n,x,y) private(i)
for (i=0; i<n; i++)
    	x[i] += y[i];
}
\end{verbatim}

\noindent A simples anotação indica para paralelizar o loop na sequência, compartilhar as variáveis $n, x$ e $y$ e manter $i$ privado. Dessa maneira simples já é possível obter ganho de desempenho utilizando os núcles da CPU. O número de \textit{threads} disparadas como \textit{default} é uma por núcleo do processador, todavia o programador pode alterar esse valor por meio da variável de ambiente OMP\_NUM\_THREAD. Para mais informações sobre OpenMP sugere-se \cite{chapman2008}. Na próxima seção será abordada a comparação entre a implementação sequencial e paralela utilizando OpenMP.

